Landmark-Guided Subgoal Generation in Hierarchical Reinforcement Learning

Goal-conditioned hierarchical reinforcement learning (HRL) has shown promising results for solving complex and long-horizon RL tasks. However, the action space of high-level policy in the goal-conditioned HRL is often large, so it results in poor exploration, leading to inefficiency in training. In this paper, we present HIerarchical reinforcement learning Guided by Landmarks (HIGL), a novel framework for training a high-level policy with a reduced action space guided by landmarks, i.e., promising states to explore. The key component of HIGL is twofold: (a) sampling landmarks that are informative for exploration and (b) encouraging the high-level policy to generate a subgoal towards a selected landmark. For (a), we consider two criteria: coverage of the entire visited state space (i.e., dispersion of states) and novelty of states (i.e., prediction error of a state). For (b), we select a landmark as the very first landmark in the shortest path in a graph whose nodes are landmarks. Our experiments demonstrate that our framework outperforms prior-arts across a variety of control tasks, thanks to efficient exploration guided by landmarks.

==> NeurIPS/2_related_works.tex <==
\section{Related work}

\paragraph{Goal-conditioned HRL.}
By introducing a hierarchy consisting of a high-level policy and a low-level policy, goal-conditioned HRL has been successful in a wide range of tasks. 
Notably, \citet{nachum2018data} proposed an off-policy correction method for goal-conditioned HRL, and 
%\citet{levy2018learning} successfully trained a policy with multiple hierarchies. 
\citet{levy2018learning} successfully trained multiple levels of policies in parallel with hindsight transitions.
% However, efficient training of a high-level policy still remains a challenge.
However, the acquisition of effective and semantically meaningful subgoals still remains a challenge.
Several works have been proposed to address this problem, including learning-based approaches \citep{dilokthanakul2019feature, ghosh2018learning, li2021learning, nachum2018near, nair2019hierarchical, nasiriany2019planning, pere2018unsupervised, sukhbaatar2018learning, vezhnevets2017feudal} and domain knowledge-based approaches \cite{nachum2018data, zhang2020generating}. The work closest to ours is HRAC \citep{zhang2020generating} that reduces the high-level action space to the $k$-adjacent region of the current state. Our work differs in that we explicitly consider the \textit{novelty} of each state within the region instead of treating all states in an equal manner.

\paragraph{Subgoal discovery.}
Identifying useful subgoals to guide training (low-level) policy has long been recognized as an effective way to solve complex RL problems \citep{mannor2004dynamic, mcgovern2001automatic, menache2002q, csimcsek2004using}. Recent works provide a subgoal by (1) constructing an environmental graph and (2) planning in the graph \citep{eysenbach2019search, huang2019mapping, laskin2020sparse, liu2020hallucinative, savinov2018semiparametric, shang2019learning, zhang2018composable, zhang2021world}. For (1), one important point is to build a graph that represents the entire map enough with a limited number of nodes. To this end, several approaches such as farthest point sampling \citep{huang2019mapping} and sparsification \citep{laskin2020sparse} were proposed. For (2), traditional planning algorithms, e.g., the Bellman-Ford algorithm, are usually used for offering the most emergent node to reach the final goal. These works have shown promising results in complex RL tasks but have a scalability issue due to increasing planning time with a larger map. Meanwhile, our framework differs from this line of works since ours ``train'' high-level policy rather than hard-coded high-level planning to generate a subgoal.

